Dark Energy Survey Year 3 results: simulation-based cosmological inference with wavelet harmonics, scattering transforms, and moments of weak lensing mass maps II. Cosmological results

We present a simulation-based cosmological analysis using a combination of Gaussian and non-Gaussian statistics of the weak lensing mass (convergence) maps from the first three years (Y3) of the Dark Energy Survey (DES). We implement: 1) second and third moments; 2) wavelet phase harmonics; 3) the scattering transform. Our analysis is fully based on simulations, spans a space of seven $\nu w$CDM cosmological parameters, and forward models the most relevant sources of systematics inherent in the data: masks, noise variations, clustering of the sources, intrinsic alignments, and shear and redshift calibration. We implement a neural network compression of the summary statistics, and we estimate the parameter posteriors using a simulation-based inference approach. Including and combining different non-Gaussian statistics is a powerful tool that strongly improves constraints over Gaussian statistics (in our case, the second moments); in particular, the Figure of Merit $\textrm{FoM}(S_8, \Omega_{\textrm{m}})$ is improved by 70 percent ($\Lambda$CDM) and 90 percent ($w$CDM). When all the summary statistics are combined, we achieve a 2 percent constraint on the amplitude of fluctuations parameter $S_8 \equiv \sigma_8 (\Omega_{\textrm{m}}/0.3)^{0.5}$, obtaining $S_8 = 0.794 \pm 0.017$ ($\Lambda$CDM) and $S_8 = 0.817 \pm 0.021$ ($w$CDM). The constraints from different statistics are shown to be internally consistent (with a $p$-value>0.1 for all combinations of statistics examined). We compare our results to other weak lensing results from the DES Y3 data, finding good consistency; we also compare with results from external datasets, such as \planck{} constraints from the Cosmic Microwave Background, finding statistical agreement, with discrepancies no greater than $<2.2\sigma$.

==> Ak.tex <==
\section*{Acknowledgements}
Funding for the DES Projects has been provided by the U.S. Department of Energy, the U.S. National Science Foundation, the Ministry of Science and Education of Spain, 
the Science and Technology Facilities Council of the United Kingdom, the Higher Education Funding Council for England, the National Center for Supercomputing 
Applications at the University of Illinois at Urbana-Champaign, the Kavli Institute of Cosmological Physics at the University of Chicago, 
the Center for Cosmology and Astro-Particle Physics at the Ohio State University,
the Mitchell Institute for Fundamental Physics and Astronomy at Texas A\&M University, Financiadora de Estudos e Projetos, 
Funda{\c c}{\~a}o Carlos Chagas Filho de Amparo {\`a} Pesquisa do Estado do Rio de Janeiro, Conselho Nacional de Desenvolvimento Cient{\'i}fico e Tecnol{\'o}gico and 
the Minist{\'e}rio da Ci{\^e}ncia, Tecnologia e Inova{\c c}{\~a}o, the Deutsche Forschungsgemeinschaft and the Collaborating Institutions in the Dark Energy Survey. 

The Collaborating Institutions are Argonne National Laboratory, the University of California at Santa Cruz, the University of Cambridge, Centro de Investigaciones Energ{\'e}ticas, 
Medioambientales y Tecnol{\'o}gicas-Madrid, the University of Chicago, University College London, the DES-Brazil Consortium, the University of Edinburgh, 
the Eidgen{\"o}ssische Technische Hochschule (ETH) Z{\"u}rich, 
Fermi National Accelerator Laboratory, the University of Illinois at Urbana-Champaign, the Institut de Ci{\`e}ncies de l'Espai (IEEC/CSIC), 
the Institut de F{\'i}sica d'Altes Energies, Lawrence Berkeley National Laboratory, the Ludwig-Maximilians Universit{\"a}t M{\"u}nchen and the associated Excellence Cluster Universe, 
the University of Michigan, NSF's NOIRLab, the University of Nottingham, The Ohio State University, the University of Pennsylvania, the University of Portsmouth, 
SLAC National Accelerator Laboratory, Stanford University, the University of Sussex, Texas A\&M University, and the OzDES Membership Consortium.

Based in part on observations at Cerro Tololo Inter-American Observatory at NSF's NOIRLab (NOIRLab Prop. ID 2012B-0001; PI: J. Frieman), which is managed by the Association of Universities for Research in Astronomy (AURA) under a cooperative agreement with the National Science Foundation.

The DES data management system is supported by the National Science Foundation under Grant Numbers AST-1138766 and AST-1536171.
The DES participants from Spanish institutions are partially supported by MICINN under grants ESP2017-89838, PGC2018-094773, PGC2018-102021, SEV-2016-0588, SEV-2016-0597, and MDM-2015-0509, some of which include ERDF funds from the European Union. IFAE is partially funded by the CERCA program of the Generalitat de Catalunya.
Research leading to these results has received funding from the European Research
Council under the European Union's Seventh Framework Program (FP7/2007-2013) including ERC grant agreements 240672, 291329, and 306478.
We  acknowledge support from the Brazilian Instituto Nacional de Ci\^encia
e Tecnologia (INCT) do e-Universo (CNPq grant 465376/2014-2).

This manuscript has been authored by Fermi Research Alliance, LLC under Contract No. DE-AC02-07CH11359 with the U.S. Department of Energy, Office of Science, Office of High Energy Physics.

\section*{Data availability}
The simulated data used in this work has been generated using the public code \texttt{FLASK} (\url{http://www.astro.iag.usp.br/~flask/}), the public T17 simulations (\url{http://cosmo.phys.hirosaki-u.ac.jp/takahasi/allsky_raytracing/}), and the public code \textsc{PKDGRAV} \citep{potter2017pkdgrav3}. The full \mcal\ catalogue will be made publicly available following publication, at the URL \url{https://des.ncsa.illinois.edu/releases}. The code used in this article will be shared on request to the corresponding author.

==> _.tex <==
@article{y3-BAOkp,
        author = {{DES Collaboration} and others},
        title = "{Dark Energy Survey Year 3 Results: BAO measurement}",
        year = "2020",
        journal = "To be submitted to ",
        }
        
@article{y3-baomocks,
        author = {{Ferraro}, I. and others},
        title = "{Dark Energy Survey Year 3 Results: Simulated Galaxy catalogues for BAO analysis}",
        year = "2020",
        journal = "To be submitted to MNRAS",
        }
        
@article{y3-baosample,
        author = {{Carnero Rosell}, A. and others},
        title = "{Dark Energy Survey Year 3 Results: Galaxy Sample for BAO Measurement}",
        year = "2020",
        journal = "To be submitted to MNRAS",
        }

@article{y3-gold,
       author = {{Sevilla-Noarbe}, I. and {Bechtol}, K. and {Carrasco Kind}, M. and {Carnero Rosell}, A. and {Becker}, M.~R. and {Drlica-Wagner}, A. and {Gruendl}, R.~A. and {Rykoff}, E.~S. and {Sheldon}, E. and {Yanny}, B. and {Alarcon}, A. and {Allam}, S. and {Amon}, A. and {Benoit-L{\'e}vy}, A. and {Bernstein}, G.~M. and {Bertin}, E. and {Burke}, D.~L. and {Carretero}, J. and {Choi}, A. and {Diehl}, H.~T. and {Everett}, S. and {Flaugher}, B. and {Gaztanaga}, E. and {Gschwend}, J. and {Harrison}, I. and {Hartley}, W.~G. and {Hoyle}, B. and {Jarvis}, M. and {Johnson}, M.~D. and {Kessler}, R. and {Kron}, R. and {Kuropatkin}, N. and {Leistedt}, B. and {Li}, T.~S. and {Menanteau}, F. and {Morganson}, E. and {Ogando}, R.~L.~C. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Pieres}, A. and {Pond}, C. and {Rodriguez-Monroy}, M. and {Smith}, J. Allyn and {Stringer}, K.~M. and {Troxel}, M.~A. and {Tucker}, D.~L. and {de Vicente}, J. and {Wester}, W. and {Zhang}, Y. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Annis}, J. and {Avila}, S. and {Bhargava}, S. and {Bridle}, S.~L. and {Brooks}, D. and {Brout}, D. and {Castander}, F.~J. and {Cawthon}, R. and {Chang}, C. and {Conselice}, C. and {Costanzi}, M. and {Crocce}, M. and {da Costa}, L.~N. and {Pereira}, M.~E.~S. and {Davis}, T.~M. and {Desai}, S. and {Dietrich}, J.~P. and {Doel}, P. and {Eckert}, K. and {Evrard}, A.~E. and {Ferrero}, I. and {Fosalba}, P. and {Garc{\'\i}a-Bellido}, J. and {Gerdes}, D.~W. and {Giannantonio}, T. and {Gruen}, D. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Huff}, E.~M. and {Huterer}, D. and {James}, D.~J. and {Jeltema}, T. and {Kuehn}, K. and {Lahav}, O. and {Lidman}, C. and {Lima}, M. and {Lin}, H. and {Maia}, M.~A.~G. and {Marshall}, J.~L. and {Martini}, P. and {Melchior}, P. and {Miquel}, R. and {Mohr}, J.~J. and {Morgan}, R. and {Neilsen}, E. and {Plazas}, A.~A. and {Romer}, A.~K. and {Roodman}, A. and {Sanchez}, E. and {Scarpine}, V. and {Schubnell}, M. and {Serrano}, S. and {Smith}, M. and {Suchyta}, E. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Varga}, T.~N. and {Wechsler}, R.~H. and {Weller}, J. and {Wilkinson}, R.~D. and {DES Collaboration}},
        title = "{Dark Energy Survey Year 3 Results: Photometric Data Set for Cosmology}",
      journal = {\apjs},
     keywords = {Surveys, Catalogs, Observational cosmology, 1671, 205, 1146, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2021,
        month = jun,
       volume = {254},
       number = {2},
          eid = {24},
        pages = {24},
          doi = {10.3847/1538-4365/abeb66},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJS..254...24S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{y3-balrog,
       author = {{Everett}, S. and {Yanny}, B. and {Kuropatkin}, N. and {Huff}, E.~M. and {Zhang}, Y. and {Myles}, J. and {Masegian}, A. and {Elvin-Poole}, J. and {Allam}, S. and {Bernstein}, G.~M. and {Sevilla-Noarbe}, I. and {Splettstoesser}, M. and {Sheldon}, E. and {Jarvis}, M. and {Amon}, A. and {Harrison}, I. and {Choi}, A. and {Hartley}, W.~G. and {Alarcon}, A. and {S{\'a}nchez}, C. and {Gruen}, D. and {Eckert}, K. and {Prat}, J. and {Tabbutt}, M. and {Busti}, V. and {Becker}, M.~R. and {MacCrann}, N. and {Diehl}, H.~T. and {Tucker}, D.~L. and {Bertin}, E. and {Jeltema}, T. and {Drlica-Wagner}, A. and {Gruendl}, R.~A. and {Bechtol}, K. and {Carnero Rosell}, A. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Annis}, J. and {Bacon}, D. and {Bhargava}, S. and {Brooks}, D. and {Burke}, D.~L. and {Carrasco Kind}, M. and {Carretero}, J. and {Castander}, F.~J. and {Conselice}, C. and {Costanzi}, M. and {da Costa}, L.~N. and {Pereira}, M.~E.~S. and {De Vicente}, J. and {DeRose}, J. and {Desai}, S. and {Eifler}, T.~F. and {Evrard}, A.~E. and {Ferrero}, I. and {Fosalba}, P. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Huterer}, D. and {James}, D.~J. and {Kent}, S. and {Krause}, E. and {Kuehn}, K. and {Lahav}, O. and {Lima}, M. and {Lin}, H. and {Maia}, M.~A.~G. and {Marshall}, J.~L. and {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Mohr}, J.~J. and {Morgan}, R. and {Muir}, J. and {Ogando}, R.~L.~C. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Plazas}, A.~A. and {Rodriguez-Monroy}, M. and {Romer}, A.~K. and {Roodman}, A. and {Sanchez}, E. and {Scarpine}, V. and {Serrano}, S. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {To}, C. and {Troxel}, M.~A. and {Varga}, T.~N. and {Weller}, J. and {Wilkinson}, R.~D.},
        title = "{Dark Energy Survey Year 3 Results: Measuring the Survey Transfer Function with Balrog}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2020,
        month = dec,
          eid = {arXiv:2012.12825},
        pages = {arXiv:2012.12825},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201212825E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{y3-deepfields,
       author = {{Hartley}, W.~G. and {Choi}, A. and {Amon}, A. and {Gruendl}, R.~A. and {Sheldon}, E. and {Harrison}, I. and {Bernstein}, G.~M. and {Sevilla-Noarbe}, I. and {Yanny}, B. and {Eckert}, K. and {Diehl}, H.~T. and {Alarcon}, A. and {Banerji}, M. and {Bechtol}, K. and {Buchs}, R. and {Cantu}, S. and {Conselice}, C. and {Cordero}, J. and {Davis}, C. and {Davis}, T.~M. and {Dodelson}, S. and {Drlica-Wagner}, A. and {Everett}, S. and {Fert{\'e}}, A. and {Gruen}, D. and {Honscheid}, K. and {Jarvis}, M. and {Johnson}, M.~D. and {Kokron}, N. and {MacCrann}, N. and {Myles}, J. and {Pace}, A.~B. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Pereira}, M.~E.~S. and {Plazas}, A.~A. and {Prat}, J. and {Rodriguez-Monroy}, M. and {Rykoff}, E.~S. and {Samuroff}, S. and {S{\'a}nchez}, C. and {Secco}, L.~F. and {Tarsitano}, F. and {Tong}, A. and {Troxel}, M.~A. and {Vasquez}, Z. and {Wang}, K. and {Zhou}, C. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Annis}, J. and {Bacon}, D. and {Bertin}, E. and {Bhargava}, S. and {Brooks}, D. and {Burke}, D.~L. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Carretero}, J. and {Castander}, F.~J. and {Costanzi}, M. and {Crocce}, M. and {da Costa}, L.~N. and {De Vicente}, J. and {DeRose}, J. and {Desai}, S. and {Dietrich}, J.~P. and {Eifler}, T.~F. and {Elvin-Poole}, J. and {Ferrero}, I. and {Flaugher}, B. and {Fosalba}, P. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Gschwend}, J. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Huterer}, D. and {James}, D.~J. and {Kent}, S. and {Krause}, E. and {Kuehn}, K. and {Kuropatkin}, N. and {Lahav}, O. and {Lin}, H. and {Maia}, M.~A.~G. and {March}, M. and {Marshall}, J.~L. and {Martini}, P. and {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Mohr}, J.~J. and {Morgan}, R. and {Neilsen}, E. and {Ogando}, R.~L.~C. and {Pandey}, S. and {Romer}, A.~K. and {Roodman}, A. and {Sako}, M. and {Sanchez}, E. and {Scarpine}, V. and {Serrano}, S. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Varga}, T.~N. and {Walker}, A.~R. and {Wester}, W. and {Wilkinson}, R.~D. and {Zuntz}, J.},
        title = "{Dark Energy Survey Year 3 Results: Deep Field Optical + Near-Infrared Images and Catalogue}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2020,
        month = dec,
          eid = {arXiv:2012.12824},
        pages = {arXiv:2012.12824},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201212824H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{y3-shapecatalog,
       author = {{Gatti}, M. and {Sheldon}, E. and {Amon}, A. and {Becker}, M. and {Troxel}, M. and {Choi}, A. and {Doux}, C. and {MacCrann}, N. and {Navarro-Alsina}, A. and {Harrison}, I. and {Gruen}, D. and {Bernstein}, G. and {Jarvis}, M. and {Secco}, L.~F. and {Fert{\'e}}, A. and {Shin}, T. and {McCullough}, J. and {Rollins}, R.~P. and {Chen}, R. and {Chang}, C. and {Pandey}, S. and {Tutusaus}, I. and {Prat}, J. and {Elvin-Poole}, J. and {Sanchez}, C. and {Plazas}, A.~A. and {Roodman}, A. and {Zuntz}, J. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Annis}, J. and {Avila}, S. and {Bacon}, D. and {Bertin}, E. and {Bhargava}, S. and {Brooks}, D. and {Burke}, D.~L. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Carretero}, J. and {Castander}, F.~J. and {Conselice}, C. and {Costanzi}, M. and {Crocce}, M. and {da Costa}, L.~N. and {Davis}, T.~M. and {De Vicente}, J. and {Desai}, S. and {Diehl}, H.~T. and {Dietrich}, J.~P. and {Doel}, P. and {Drlica-Wagner}, A. and {Eckert}, K. and {Everett}, S. and {Ferrero}, I. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gerdes}, D.~W. and {Giannantonio}, T. and {Gruendl}, R.~A. and {Gschwend}, J. and {Gutierrez}, G. and {Hartley}, W.~G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Hoyle}, B. and {Huff}, E.~M. and {Huterer}, D. and {Jain}, B. and {James}, D.~J. and {Jeltema}, T. and {Krause}, E. and {Kron}, R. and {Kuropatkin}, N. and {Lima}, M. and {Maia}, M.~A.~G. and {Marshall}, J.~L. and {Miquel}, R. and {Morgan}, R. and {Myles}, J. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Rykoff}, E.~S. and {Samuroff}, S. and {Sanchez}, E. and {Scarpine}, V. and {Schubnell}, M. and {Serrano}, S. and {Sevilla-Noarbe}, I. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Tucker}, D.~L. and {Varga}, T.~N. and {Wechsler}, R.~H. and {Weller}, J. and {Wester}, W. and {Wilkinson}, R.~D.},
        title = "{Dark energy survey year 3 results: weak lensing shape catalogue}",
      journal = {\mnras},
     keywords = {gravitational lensing: weak, methods: data analysis, techniques: image processing, catalogues, surveys, cosmology: observations, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = jul,
       volume = {504},
       number = {3},
        pages = {4312-4336},
          doi = {10.1093/mnras/stab918},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.504.4312G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{y3-piff,
       author = {{Jarvis}, M. and {Bernstein}, G.~M. and {Amon}, A. and {Davis}, C. and {L{\'e}get}, P.~F. and {Bechtol}, K. and {Harrison}, I. and {Gatti}, M. and {Roodman}, A. and {Chang}, C. and {Chen}, R. and {Choi}, A. and {Desai}, S. and {Drlica-Wagner}, A. and {Gruen}, D. and {Gruendl}, R.~A. and {Hernandez}, A. and {MacCrann}, N. and {Meyers}, J. and {Navarro-Alsina}, A. and {Pandey}, S. and {Plazas}, A.~A. and {Secco}, L.~F. and {Sheldon}, E. and {Troxel}, M.~A. and {Vorperian}, S. and {Wei}, K. and {Zuntz}, J. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Avila}, S. and {Bhargava}, S. and {Bridle}, S.~L. and {Brooks}, D. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Carretero}, J. and {Costanzi}, M. and {da Costa}, L.~N. and {De Vicente}, J. and {Diehl}, H.~T. and {Doel}, P. and {Everett}, S. and {Flaugher}, B. and {Fosalba}, P. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {James}, D.~J. and {Kent}, S. and {Kuehn}, K. and {Kuropatkin}, N. and {Lahav}, O. and {Maia}, M.~A.~G. and {March}, M. and {Marshall}, J.~L. and {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Ogando}, R.~L.~C. and {Paz-Chinch{\'o}n}, F. and {Rykoff}, E.~S. and {Sanchez}, E. and {Scarpine}, V. and {Schubnell}, M. and {Serrano}, S. and {Sevilla-Noarbe}, I. and {Smith}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {Varga}, T.~N. and {Walker}, A.~R. and {Wester}, W. and {Wilkinson}, R.~D. and {DES Collaboration}},
        title = "{Dark Energy Survey year 3 results: point spread function modelling}",
      journal = {\mnras},
     keywords = {gravitational lensing: weak, techniques: image processing, catalogues, surveys, software: data analysis, cosmology: observations, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = feb,
       volume = {501},
       number = {1},
        pages = {1282-1299},
          doi = {10.1093/mnras/staa3679},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.501.1282J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{y3-imagesims,
       author = {{MacCrann}, N. and {Becker}, M.~R. and {McCullough}, J. and {Amon}, A. and {Gruen}, D. and {Jarvis}, M. and {Choi}, A. and {Troxel}, M.~A. and {Sheldon}, E. and {Yanny}, B. and {Herner}, K. and {Dodelson}, S. and {Zuntz}, J. and {Eckert}, K. and {Rollins}, R.~P. and {Varga}, T.~N. and {Bernstein}, G.~M. and {Gruendl}, R.~A. and {Harrison}, I. and {Hartley}, W.~G. and {Sevilla-Noarbe}, I. and {Pieres}, A. and {Bridle}, S.~L. and {Myles}, J. and {Alarcon}, A. and {Everett}, S. and {S{\'a}nchez}, C. and {Huff}, E.~M. and {Tarsitano}, F. and {Gatti}, M. and {Secco}, L.~F. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Annis}, J. and {Bacon}, D. and {Bertin}, E. and {Brooks}, D. and {Burke}, D.~L. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Carretero}, J. and {Costanzi}, M. and {Crocce}, M. and {Pereira}, M.~E.~S. and {De Vicente}, J. and {Desai}, S. and {Diehl}, H.~T. and {Dietrich}, J.~P. and {Doel}, P. and {Eifler}, T.~F. and {Ferrero}, I. and {Fert{\'e}}, A. and {Flaugher}, B. and {Fosalba}, P. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Giannantonio}, T. and {Gschwend}, J. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {James}, D.~J. and {Lahav}, O. and {Lima}, M. and {Maia}, M.~A.~G. and {March}, M. and {Marshall}, J.~L. and {Martini}, P. and {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Mohr}, J.~J. and {Morgan}, R. and {Muir}, J. and {Ogando}, R.~L.~C. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Plazas}, A.~A. and {Rodriguez-Monroy}, M. and {Roodman}, A. and {Samuroff}, S. and {Sanchez}, E. and {Scarpine}, V. and {Serrano}, S. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Wilkinson}, R.~D.},
        title = "{DES Y3 results: Blending shear and redshift biases in image simulations}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = dec,
          eid = {arXiv:2012.08567},
        pages = {arXiv:2012.08567},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201208567M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{y3-sompz,
author = {{Myles}, J. and {Alarcon}, A. and {Amon}, A. and {S{\'a}nchez}, C. and {Everett}, S. and {DeRose}, J. and {McCullough}, J. and {Gruen}, D. and {Bernstein}, G.~M. and {Troxel}, M.~A. and {Dodelson}, S. and {Campos}, A. and {MacCrann}, N. and {Yin}, B. and {Raveri}, M. and {Amara}, A. and {Becker}, M.~R. and {Choi}, A. and {Cordero}, J. and {Eckert}, K. and {Gatti}, M. and {Giannini}, G. and {Gschwend}, J. and {Gruendl}, R.~A. and {Harrison}, I. and {Hartley}, W.~G. and {Huff}, E.~M. and {Kuropatkin}, N. and {Lin}, H. and {Masters}, D. and {Miquel}, R. and {Prat}, J. and {Roodman}, A. and {Rykoff}, E.~S. and {Sevilla-Noarbe}, I. and {Sheldon}, E. and {Wechsler}, R.~H. and {Yanny}, B. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Annis}, J. and {Bacon}, D. and {Bertin}, E. and {Bhargava}, S. and {Bridle}, S.~L. and {Brooks}, D. and {Burke}, D.~L. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Carretero}, J. and {Castander}, F.~J. and {Conselice}, C. and {Costanzi}, M. and {Crocce}, M. and {da Costa}, L.~N. and {Pereira}, M.~E.~S. and {Desai}, S. and {Diehl}, H.~T. and {Eifler}, T.~F. and {Elvin-Poole}, J. and {Evrard}, A.~E. and {Ferrero}, I. and {Fert{\'e}}, A. and {Flaugher}, B. and {Fosalba}, P. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Giannantonio}, T. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Hoyle}, B. and {Huterer}, D. and {James}, D.~J. and {Krause}, E. and {Kuehn}, K. and {Lahav}, O. and {Lima}, M. and {Maia}, M.~A.~G. and {Marshall}, J.~L. and {Martini}, P. and {Melchior}, P. and {Menanteau}, F. and {Mohr}, J.~J. and {Morgan}, R. and {Muir}, J. and {Ogando}, R.~L.~C. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Plazas}, A.~A. and {Rodriguez-Monroy}, M. and {Samuroff}, S. and {Sanchez}, E. and {Scarpine}, V. and {Secco}, L.~F. and {Serrano}, S. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Varga}, T.~N. and {Weller}, J. and {Wester}, W.},
        title = "{Dark Energy Survey Year 3 results: redshift calibration of the weak lensing source galaxies}",
      journal = {\mnras},
     keywords = {gravitational lensing: weak, galaxies: distances and redshifts, dark energy, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = aug,
       volume = {505},
       number = {3},
        pages = {4249-4277},
          doi = {10.1093/mnras/stab1515},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.505.4249M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{y3-sourcewz,
       author = {{Gatti}, M. and {Giannini}, G. and {Bernstein}, G.~M. and {Alarcon}, A. and {Myles}, J. and {Amon}, A. and {Cawthon}, R. and {Troxel}, M. and {DeRose}, J. and {Everett}, S. and {Ross}, A.~J. and {Rykoff}, E.~S. and {Elvin-Poole}, J. and {Cordero}, J. and {Harrison}, I. and {Sanchez}, C. and {Prat}, J. and {Gruen}, D. and {Lin}, H. and {Crocce}, M. and {Rozo}, E. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Annis}, J. and {Avila}, S. and {Bacon}, D. and {Bertin}, E. and {Brooks}, D. and {Burke}, D.~L. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Carretero}, J. and {Castander}, F.~J. and {Choi}, A. and {Conselice}, C. and {Costanzi}, M. and {Crocce}, M. and {da Costa}, L.~N. and {Pereira}, M.~E.~S. and {Dawson}, K. and {Desai}, S. and {Diehl}, H.~T. and {Eckert}, K. and {Eifler}, T.~F. and {Evrard}, A.~E. and {Ferrero}, I. and {Flaugher}, B. and {Fosalba}, P. and {Frieman}, J. and {Garcia-Bellido}, J. and {Gaztanaga}, E. and {Giannantonio}, T. and {Gruendl}, R.~A. and {Gschwend}, J. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Hoyle}, B. and {Huterer}, D. and {James}, D.~J. and {Kuehn}, K. and {Kuropatkin}, N. and {Lahav}, O. and {Lima}, M. and {MacCrann}, N. and {Maia}, M.~A.~G. and {March}, M. and {Marshall}, J.~L. and {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Mohr}, J.~J. and {Morgan}, R. and {Ogando}, R.~L.~C. and {Palmese}, A. and {Paz-Chinchon}, F. and {Percival}, W.~J. and {Plazas}, A.~A. and {Rodriguez-Monroy}, M. and {Roodman}, A. and {Rossi}, G. and {Samuroff}, S. and {Sanchez}, E. and {Scarpine}, V. and {Secco}, L.~F. and {Serrano}, S. and {Sevilla-Noarbe}, I. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Varga}, T.~N. and {Weller}, J. and {Wilkinson}, R.~D.},
        title = "{Dark Energy Survey Year 3 Results: Clustering Redshifts -- Calibration of the Weak Lensing Source Redshift Distributions with redMaGiC and BOSS/eBOSS}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = dec,
          eid = {arXiv:2012.08569},
        pages = {arXiv:2012.08569},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201208569G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{y3-lenswz,
       author = {{Cawthon}, R. and {Elvin-Poole}, J. and {Porredon}, A. and {Crocce}, M. and {Giannini}, G. and {Gatti}, M. and {Ross}, A.~J. and {Rykoff}, E.~S. and {Carnero Rosell}, A. and {DeRose}, J. and {Lee}, S. and {Rodriguez-Monroy}, M. and {Amon}, A. and {Bechtol}, K. and {De Vicente}, J. and {Gruen}, D. and {Morgan}, R. and {Sanchez}, E. and {Sanchez}, J. and {Sevilla-Noarbe}, I. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Annis}, J. and {Avila}, S. and {Bacon}, D. and {Bertin}, E. and {Brooks}, D. and {Burke}, D.~L. and {Carrasco Kind}, M. and {Carretero}, J. and {Castander}, F.~J. and {Choi}, A. and {Costanzi}, M. and {da Costa}, L.~N. and {Pereira}, M.~E.~S. and {Dawson}, K. and {Desai}, S. and {Diehl}, H.~T. and {Eckert}, K. and {Everett}, S. and {Ferrero}, I. and {Fosalba}, P. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gruendl}, R.~A. and {Gschwend}, J. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Huterer}, D. and {James}, D.~J. and {Kim}, A.~G. and {Kneib}, J. -P. and {Kuehn}, K. and {Kuropatkin}, N. and {Lahav}, O. and {Lima}, M. and {Lin}, H. and {Maia}, M.~A.~G. and {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Mohr}, J.~J. and {Muir}, J. and {Myles}, J. and {Palmese}, A. and {Pandey}, S. and {Paz-Chinch{\'o}n}, F. and {Percival}, W.~J. and {Plazas}, A.~A. and {Roodman}, A. and {Rossi}, G. and {Scarpine}, V. and {Serrano}, S. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {To}, C. and {Troxel}, M.~A. and {Wilkinson}, R.~D. and {the DES Collaboration}},
        title = "{Dark Energy Survey Year 3 Results: Calibration of Lens Sample Redshift Distributions using Clustering Redshifts with BOSS/eBOSS}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = dec,
          eid = {arXiv:2012.12826},
        pages = {arXiv:2012.12826},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201212826C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{y3-sompzbuzzard,
       author = {{Buchs}, R. and {Davis}, C. and {Gruen}, D. and {DeRose}, J. and
         {Alarcon}, A. and {Bernstein}, G.~M. and {S{\'a}nchez}, C. and
         {Myles}, J. and {Roodman}, A. and {Allen}, S. and {Amon}, A. and
         {Choi}, A. and {Masters}, D.~C. and {Miquel}, R. and {Troxel}, M.~A. and
         {Wechsler}, R.~H. and {Abbott}, T.~M.~C. and {Annis}, J. and
         {Avila}, S. and {Bechtol}, K. and {Bridle}, S.~L. and {Brooks}, D. and
         {Buckley-Geer}, E. and {Burke}, D.~L. and {Carnero Rosell}, A. and
         {Carrasco Kind}, M. and {Carretero}, J. and {Castander}, F.~J. and
         {Cawthon}, R. and {D'Andrea}, C.~B. and {da Costa}, L.~N. and
         {De Vicente}, J. and {Desai}, S. and {Diehl}, H.~T. and {Doel}, P. and
         {Drlica-Wagner}, A. and {Eifler}, T.~F. and {Evrard}, A.~E. and
         {Flaugher}, B. and {Fosalba}, P. and {Frieman}, J. and
         {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gruendl}, R.~A. and
         {Gschwend}, J. and {Gutierrez}, G. and {Hartley}, W.~G. and
         {Hollowood}, D.~L. and {Honscheid}, K. and {James}, D.~J. and
         {Kuehn}, K. and {Kuropatkin}, N. and {Lima}, M. and {Lin}, H. and
         {Maia}, M.~A.~G. and {March}, M. and {Marshall}, J.~L. and
         {Melchior}, P. and {Menanteau}, F. and {Ogando}, R.~L.~C. and
         {Plazas}, A.~A. and {Rykoff}, E.~S. and {Sanchez}, E. and
         {Scarpine}, V. and {Serrano}, S. and {Sevilla-Noarbe}, I. and
         {Smith}, M. and {Soares-Santos}, M. and {Sobreira}, F. and
         {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {Thomas}, D. and
         {Vikram}, V. and {DES Collaboration}},
        title = "{Phenotypic redshifts with self-organizing maps: A novel method to characterize redshift distributions of source galaxies for weak lensing}",
      journal = {\mnras},
     keywords = {gravitational lensing: weak, galaxies: distances and redshifts, dark energy, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = oct,
       volume = {489},
       number = {1},
        pages = {820-841},
          doi = {10.1093/mnras/stz2162},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.489..820B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{y3-hyperrank,
        author = {{Cordero}, Juan P. and {Harrison}, Ian and {Rollins}, Richard P. and {Bernstein}, G.~M. and {Bridle}, S.~L. and {Alarcon}, A. and {Alves}, O. and {Amon}, A. and {Andrade-Oliveira}, F. and {Camacho}, H. and {Campos}, A. and {Choi}, A. and {DeRose}, J. and {Dodelson}, S. and {Eckert}, K. and {Eifler}, T.~F. and {Everett}, S. and {Fang}, X. and {Friedrich}, O. and {Gruen}, D. and {Gruendl}, R.~A. and {Hartley}, W.~G. and {Huff}, E.~M. and {Krause}, E. and {Kuropatkin}, N. and {MacCrann}, N. and {McCullough}, J. and {Myles}, J. and {Pandey}, S. and {Raveri}, M. and {Rosenfeld}, R. and {Rykoff}, E.~S. and {S{\'a}nchez}, C. and {S{\'a}nchez}, J. and {Sevilla-Noarbe}, I. and {Sheldon}, E. and {Troxel}, M. and {Wechsler}, R. and {Yanny}, B. and {Yin}, B. and {Zhang}, Y. and {Aguena}, M. and {Allam}, S. and {Bertin}, E. and {Brooks}, D. and {Burke}, D.~L. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Carretero}, J. and {Castander}, F.~J. and {Cawthon}, R. and {Costanzi}, M. and {da Costa}, L. and {da Silva Pereira}, M.~E. and {De Vicente}, J. and {Diehl}, H.~T. and {Dietrich}, J. and {Doel}, P. and {Elvin-Poole}, J. and {Ferrero}, I. and {Flaugher}, B. and {Fosalba}, P. and {Frieman}, J. and {Garcia-Bellido}, J. and {Gerdes}, D. and {Gschwend}, J. and {Gutierrez}, G. and {Hinton}, S. and {Hollowood}, D.~L. and {Honscheid}, K. and {Hoyle}, B. and {James}, D. and {Kuehn}, K. and {Lahav}, O. and {Maia}, M.~A.~G. and {March}, M. and {Menanteau}, F. and {Miquel}, R. and {Morgan}, R. and {Muir}, J. and {Palmese}, A. and {Paz-Chinchon}, F. and {Pieres}, A. and {Plazas Malag{\'o}n}, A. and {S{\'a}nchez}, E. and {Scarpine}, V. and {Serrano}, S. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Varga}, T.~N.},
        title = "{Dark Energy Survey Year 3 results: Marginalisation over redshift distribution uncertainties using ranking of discrete realisations}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = sep,
          eid = {arXiv:2109.09636},
        pages = {arXiv:2109.09636},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210909636C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{y3-shearratio,
        author = {{S{\'a}nchez}, C. and {Prat}, J. and {Zacharegkas}, G. and {Pandey}, S. and {Baxter}, E. and {Bernstein}, G.~M. and {Blazek}, J. and {Cawthon}, R. and {Chang}, C. and {Krause}, E. and {Lemos}, P. and {Park}, Y. and {Raveri}, M. and {Sanchez}, J. and {Troxel}, M.~A. and {Amon}, A. and {Fang}, X. and {Friedrich}, O. and {Gruen}, D. and {Porredon}, A. and {Secco}, L.~F. and {Samuroff}, S. and {Alarcon}, A. and {Alves}, O. and {Andrade-Oliveira}, F. and {Bechtol}, K. and {Becker}, M.~R. and {Camacho}, H. and {Campos}, A. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Chen}, R. and {Choi}, A. and {Crocce}, M. and {Davis}, C. and {De Vicente}, J. and {DeRose}, J. and {Di Valentino}, E. and {Diehl}, H.~T. and {Dodelson}, S. and {Doux}, C. and {Drlica-Wagner}, A. and {Eckert}, K. and {Eifler}, T.~F. and {Elsner}, F. and {Elvin-Poole}, J. and {Everett}, S. and {Fert{\'e}}, A. and {Fosalba}, P. and {Gatti}, M. and {Giannini}, G. and {Gruendl}, R.~A. and {Harrison}, I. and {Hartley}, W.~G. and {Herner}, K. and {Huff}, E.~M. and {Huterer}, D. and {Jarvis}, M. and {Jain}, B. and {Kuropatkin}, N. and {Leget}, P. -F. and {MacCrann}, N. and {McCullough}, J. and {Muir}, J. and {Myles}, J. and {Navarro-Alsina}, A. and {Rollins}, R.~P. and {Roodman}, A. and {Rosenfeld}, R. and {Rykoff}, E.~S. and {Sevilla-Noarbe}, I. and {Sheldon}, E. and {Shin}, T. and {Troja}, A. and {Tutusaus}, I. and {Varga}, T.~N. and {Wechsler}, R.~H. and {Yanny}, B. and {Yin}, B. and {Zhang}, Y. and {Zuntz}, J. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Bacon}, D. and {Bertin}, E. and {Bhargava}, S. and {Brooks}, D. and {Buckley-Geer}, E. and {Burke}, D.~L. and {Carretero}, J. and {Costanzi}, M. and {da Costa}, L.~N. and {Pereira}, M.~E.~S. and {Desai}, S. and {Dietrich}, J.~P. and {Doel}, P. and {Evrard}, A.~E. and {Ferrero}, I. and {Flaugher}, B. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Giannantonio}, T. and {Gschwend}, J. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Hoyle}, B. and {James}, D.~J. and {Kuehn}, K. and {Lahav}, O. and {Lima}, M. and {Lin}, H. and {Maia}, M.~A.~G. and {Marshall}, J.~L. and {Martini}, P. and {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Mohr}, J.~J. and {Morgan}, R. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Petravick}, D. and {Pieres}, A. and {Plazas Malag{\'o}n}, A.~A. and {Rodriguez-Monroy}, M. and {Sanchez}, E. and {Scarpine}, V. and {Schubnell}, M. and {Serrano}, S. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {Thomas}, D. and {To}, C.},
        title = "{Dark Energy Survey Year 3 Results: Exploiting small-scale information with lensing shear ratios}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = may,
          eid = {arXiv:2105.13542},
        pages = {arXiv:2105.13542},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210513542S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{y3-simvalidation,
        author = {{DeRose}, J. and others},
        title = "{Dark Energy Survey Year 3 Results: Validating $3\times2$-point Modeling and Analysis Choices using Cosmological Simulations}",
        year = "2021",
        journal = "To be submitted to ",
        }

@article{y3-samplers,
        author = {{Surname}, A. and others},
        title = "{Dark Energy Survey Year 3 Results: }",
        year = "2020",
        journal = "To be submitted to ",
        }

@article{y3-tensions,
       author = {{Lemos}, P. and {Raveri}, M. and {Campos}, A. and {Park}, Y. and {Chang}, C. and {Weaverdyck}, N. and {Huterer}, D. and {Liddle}, A.~R. and {Blazek}, J. and {Cawthon}, R. and {Choi}, A. and {DeRose}, J. and {Dodelson}, S. and {Doux}, C. and {Gatti}, M. and {Gruen}, D. and {Harrison}, I. and {Krause}, E. and {Lahav}, O. and {MacCrann}, N. and {Muir}, J. and {Prat}, J. and {Rau}, M.~M. and {Rollins}, R.~P. and {Samuroff}, S. and {Zuntz}, J. and {Hartley}, W.~G. and {Hoyle}, B. and {Sevilla-Noarbe}, I. and {Troxel}, M.~A. and {Aguena}, M. and {Allam}, S. and {Annis}, J. and {Avila}, S. and {Bacon}, D. and {Bernstein}, G.~M. and {Bertin}, E. and {Brooks}, D. and {Burke}, D.~L. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Carretero}, J. and {Conselice}, C. and {Costanzi}, M. and {Crocce}, M. and {Pereira}, M.~E.~S. and {De Vicente}, J. and {Desai}, S. and {Diehl}, H.~T. and {Doel}, P. and {Eckert}, K. and {Eifler}, T.~F. and {Elvin-Poole}, J. and {Everett}, S. and {Evrard}, A.~E. and {Ferrero}, I. and {Fert{\'e}}, A. and {Flaugher}, B. and {Fosalba}, P. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Giannantonio}, T. and {Gruendl}, R.~A. and {Gschwend}, J. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Huff}, E.~M. and {James}, D.~J. and {Jarvis}, M. and {Lima}, M. and {Maia}, M.~A.~G. and {March}, M. and {Marshall}, J.~L. and {Martini}, P. and {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Mohr}, J.~J. and {Morgan}, R. and {Myles}, J. and {Ogando}, R.~L.~C. and {Palmese}, A. and {Pandey}, S. and {Paz-Chinch{\'o}n}, F. and {Plazas}, A.~A. and {Rodriguez-Monroy}, M. and {Roodman}, A. and {Sanchez}, E. and {Scarpine}, V. and {Schubnell}, M. and {Secco}, L.~F. and {Serrano}, S. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Varga}, T.~N. and {Weller}, J. and {Wester}, W.},
        title = "{Assessing tension metrics with Dark Energy Survey and Planck data}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2020,
        month = dec,
          eid = {arXiv:2012.09554},
        pages = {arXiv:2012.09554},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201209554L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{y3-inttensions,
       author = {{Doux}, C. and {Baxter}, E. and {Lemos}, P. and {Chang}, C. and {Alarcon}, A. and {Amon}, A. and {Campos}, A. and {Choi}, A. and {Gatti}, M. and {Gruen}, D. and {Jarvis}, M. and {MacCrann}, N. and {Park}, Y. and {Prat}, J. and {Rau}, M.~M. and {Raveri}, M. and {Samuroff}, S. and {DeRose}, J. and {Hartley}, W.~G. and {Hoyle}, B. and {Troxel}, M.~A. and {Zuntz}, J. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Annis}, J. and {Avila}, S. and {Bacon}, D. and {Bertin}, E. and {Bhargava}, S. and {Brooks}, D. and {Burke}, D.~L. and {Carrasco Kind}, M. and {Carretero}, J. and {Cawthon}, R. and {Costanzi}, M. and {da Costa}, L.~N. and {Pereira}, M.~E.~S. and {Desai}, S. and {Diehl}, H.~T. and {Dietrich}, J.~P. and {Doel}, P. and {Everett}, S. and {Ferrero}, I. and {Fosalba}, P. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gerdes}, D.~W. and {Giannantonio}, T. and {Gruendl}, R.~A. and {Gschwend}, J. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Huff}, E.~M. and {Huterer}, D. and {Jain}, B. and {James}, D.~J. and {Krause}, E. and {Kuehn}, K. and {Kuropatkin}, N. and {Lahav}, O. and {Lidman}, C. and {Lima}, M. and {Maia}, M.~A.~G. and {Menanteau}, F. and {Miquel}, R. and {Morgan}, R. and {Muir}, J. and {Ogando}, R.~L.~C. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Plazas}, A.~A. and {Sanchez}, E. and {Scarpine}, V. and {Schubnell}, M. and {Serrano}, S. and {Sevilla-Noarbe}, I. and {Smith}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {To}, C. and {Tucker}, D.~L. and {Varga}, T.~N. and {Weller}, J. and {Wilkinson}, R.~D.},
        title = "{Dark energy survey internal consistency tests of the joint cosmological probes analysis with posterior predictive distributions}",
      journal = {\mnras},
     keywords = {gravitational lensing: weak, methods: statistical, dark energy, large-scale structure of Universe, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2021,
        month = may,
       volume = {503},
       number = {2},
        pages = {2688-2705},
          doi = {10.1093/mnras/stab526},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.503.2688D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{y3-covariances,
       author = {{Friedrich}, O. and {Andrade-Oliveira}, F. and {Camacho}, H. and {Alves}, O. and {Rosenfeld}, R. and {Sanchez}, J. and {Fang}, X. and {Eifler}, T.~F. and {Krause}, E. and {Chang}, C. and {Omori}, Y. and {Amon}, A. and {Baxter}, E. and {Elvin-Poole}, J. and {Huterer}, D. and {Porredon}, A. and {Prat}, J. and {Terra}, V. and {Troja}, A. and {Alarcon}, A. and {Bechtol}, K. and {Bernstein}, G.~M. and {Buchs}, R. and {Campos}, A. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Cawthon}, R. and {Choi}, A. and {Cordero}, J. and {Crocce}, M. and {Davis}, C. and {DeRose}, J. and {Diehl}, H.~T. and {Dodelson}, S. and {Doux}, C. and {Drlica-Wagner}, A. and {Elsner}, F. and {Everett}, S. and {Fosalba}, P. and {Gatti}, M. and {Giannini}, G. and {Gruen}, D. and {Gruendl}, R.~A. and {Harrison}, I. and {Hartley}, W.~G. and {Jain}, B. and {Jarvis}, M. and {MacCrann}, N. and {McCullough}, J. and {Muir}, J. and {Myles}, J. and {Pandey}, S. and {Raveri}, M. and {Roodman}, A. and {Rodriguez-Monroy}, M. and {Rykoff}, E.~S. and {Samuroff}, S. and {S{\'a}nchez}, C. and {Secco}, L.~F. and {Sevilla-Noarbe}, I. and {Sheldon}, E. and {Troxel}, M.~A. and {Weaverdyck}, N. and {Yanny}, B. and {Aguena}, M. and {Avila}, S. and {Bacon}, D. and {Bertin}, E. and {Bhargava}, S. and {Brooks}, D. and {Burke}, D.~L. and {Carretero}, J. and {Costanzi}, M. and {da Costa}, L.~N. and {Pereira}, M.~E.~S. and {De Vicente}, J. and {Desai}, S. and {Evrard}, A.~E. and {Ferrero}, I. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Giannantonio}, T. and {Gschwend}, J. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {James}, D.~J. and {Kuehn}, K. and {Lahav}, O. and {Lima}, M. and {Maia}, M.~A.~G. and {Menanteau}, F. and {Miquel}, R. and {Morgan}, R. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Plazas}, A.~A. and {Sanchez}, E. and {Scarpine}, V. and {Serrano}, S. and {Soares-Santos}, M. and {Smith}, M. and {Suchyta}, E. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Varga}, T.~N. and {Weller}, J. and {Wilkinson}, R.~D.},
        title = "{Dark Energy Survey Year 3 Results: Covariance Modelling and its Impact on Parameter Estimation and Quality of Fit}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = dec,
          eid = {arXiv:2012.08568},
        pages = {arXiv:2012.08568},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201208568F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{y3-blinding,
       author = {{Muir}, J. and {Bernstein}, G.~M. and {Huterer}, D. and {Elsner}, F. and
         {Krause}, E. and {Roodman}, A. and {Allam}, S. and {Annis}, J. and
         {Avila}, S. and {Bechtol}, K. and {Bertin}, E. and {Brooks}, D. and
         {Buckley-Geer}, E. and {Burke}, D.~L. and {Carnero Rosell}, A. and
         {Carrasco Kind}, M. and {Carretero}, J. and {Cawthon}, R. and
         {Costanzi}, M. and {da Costa}, L.~N. and {De Vicente}, J. and
         {Desai}, S. and {Dietrich}, J.~P. and {Doel}, P. and {Eifler}, T.~F. and
         {Everett}, S. and {Fosalba}, P. and {Frieman}, J. and
         {Garc{\'\i}a-Bellido}, J. and {Gerdes}, D.~W. and {Gruen}, D. and
         {Gruendl}, R.~A. and {Gschwend}, J. and {Hartley}, W.~G. and
         {Hollowood}, D.~L. and {James}, D.~J. and {Jarvis}, M. and {Kuehn}, K. and
         {Kuropatkin}, N. and {Lahav}, O. and {March}, M. and {Marshall}, J.~L. and
         {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Ogand
        o}, R.~L.~C. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and
         {Plazas}, A.~A. and {Romer}, A.~K. and {Sanchez}, E. and
         {Scarpine}, V. and {Schubnell}, M. and {Serrano}, S. and
         {Sevilla-Noarbe}, I. and {Smith}, M. and {Suchyta}, E. and {Tarle}, G. and
         {Thomas}, D. and {Troxel}, M.~A. and {Walker}, A.~R. and {Weller}, J. and
         {Wester}, W. and {Zuntz}, J. and {DES Collaboration}},
        title = "{Blinding multiprobe cosmological experiments}",
      journal = {\mnras},
     keywords = {methods: data analysis, methods: numerical, methods: statistical, cosmology: observations; large-scale structure of Universe, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2020,
        month = apr,
       volume = {494},
       number = {3},
        pages = {4454-4470},
          doi = {10.1093/mnras/staa965},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.494.4454M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{y3-generalmethods,
        author = {{Krause}, E. and others},
        title = "{Dark Energy Survey Year 3 Results: Multi-probe modeling validation}",
        year = "2021",
        journal = "To be submitted to MNRAS",
        }

@article{y3-massmapping,
        author = {{Jeffrey}, N. and {Gatti}, M. and {Chang}, C. and {Whiteway}, L. and {Demirbozan}, U. and {Kovacs}, A. and {Pollina}, G. and {Bacon}, D. and {Hamaus}, N. and {Kacprzak}, T. and {Lahav}, O. and {Lanusse}, F. and {Mawdsley}, B. and {Nadathur}, S. and {Starck}, J.~L. and {Vielzeuf}, P. and {Zeurcher}, D. and {Alarcon}, A. and {Amon}, A. and {Bechtol}, K. and {Bernstein}, G.~M. and {Campos}, A. and {Rosell}, A. Carnero and {Kind}, M. Carrasco and {Cawthon}, R. and {Chen}, R. and {Choi}, A. and {Cordero}, J. and {Davis}, C. and {DeRose}, J. and {Doux}, C. and {Drlica-Wagner}, A. and {Eckert}, K. and {Elsner}, F. and {Elvin-Poole}, J. and {Everett}, S. and {Fert{\'e}}, A. and {Giannini}, G. and {Gruen}, D. and {Gruendl}, R.~A. and {Harrison}, I. and {Hartley}, W.~G. and {Herner}, K. and {Huff}, E.~M. and {Huterer}, D. and {Kuropatkin}, N. and {Jarvis}, M. and {Leget}, P.~F. and {MacCrann}, N. and {McCullough}, J. and {Muir}, J. and {Myles}, J. and {Navarro-Alsina}, A. and {Pandey}, S. and {Prat}, J. and {Raveri}, M. and {Rollins}, R.~P. and {Ross}, A.~J. and {Rykoff}, E.~S. and {S{\'a}nchez}, C. and {Secco}, L.~F. and {Sevilla-Noarbe}, I. and {Sheldon}, E. and {Shin}, T. and {Troxel}, M.~A. and {Tutusaus}, I. and {Varga}, T.~N. and {Yanny}, B. and {Yin}, B. and {Zhang}, Y. and {Zuntz}, J. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Andrade-Oliveira}, F. and {Becker}, M.~R. and {Bertin}, E. and {Bhargava}, S. and {Brooks}, D. and {Burke}, D.~L. and {Carretero}, J. and {Castander}, F.~J. and {Conselice}, C. and {Costanzi}, M. and {Crocce}, M. and {da Costa}, L.~N. and {Pereira}, M.~E.~S. and {De Vicente}, J. and {Desai}, S. and {Diehl}, H.~T. and {Dietrich}, J.~P. and {Doel}, P. and {Ferrero}, I. and {Flaugher}, B. and {Fosalba}, P. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Giannantonio}, T. and {Gschwend}, J. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Hoyle}, B. and {Jain}, B. and {James}, D.~J. and {Lima}, M. and {Maia}, M.~A.~G. and {March}, M. and {Marshall}, J.~L. and {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Mohr}, J.~J. and {Morgan}, R. and {Ogando}, R.~L.~C. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Plazas}, A.~A. and {Rodriguez-Monroy}, M. and {Roodman}, A. and {Sanchez}, E. and {Scarpine}, V. and {Serrano}, S. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Weller}, J. and {DES Collaboration}},
        title = "{Dark Energy Survey Year 3 results: Curved-sky weak lensing mass map reconstruction}",
      journal = {\mnras},
     keywords = {gravitational lensing: weak, methods: statistical, large-scale structure of Universe, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = aug,
       volume = {505},
       number = {3},
        pages = {4626-4645},
          doi = {10.1093/mnras/stab1495},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.505.4626J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{y3-galaxyclustering,
        author = {{Rodr\'iguez-Monroy}, M. and others},
        title = "{Dark Energy Survey Year 3 Results: Galaxy clustering and systematics treatment for lens galaxy samples}",
        year = "2021",
        journal = "To be submitted to MNRAS",
        }

@article{y3-gglensing,
        author = {{Prat}, J. and others},
        title = "{Dark Energy Survey Year 3 Results: Accurate measurement and modeling of galaxy-galaxy lensing}",
        year = "2021",
        journal = "To be submitted to MNRAS",
        }

@article{y3-cosmicshear1,
        author = {{Amon}, A. and {Gruen}, D. and {Troxel}, M.~A. and {MacCrann}, N. and {Dodelson}, S. and {Choi}, A. and {Doux}, C. and {Secco}, L.~F. and {Samuroff}, S. and {Krause}, E. and {Cordero}, J. and {Myles}, J. and {DeRose}, J. and {Wechsler}, R.~H. and {Gatti}, M. and {Navarro-Alsina}, A. and {Bernstein}, G.~M. and {Jain}, B. and {Blazek}, J. and {Alarcon}, A. and {Fert{\'e}}, A. and {Raveri}, M. and {Lemos}, P. and {Campos}, A. and {Prat}, J. and {S{\'a}nchez}, C. and {Jarvis}, M. and {Alves}, O. and {Andrade-Oliveira}, F. and {Baxter}, E. and {Bechtol}, K. and {Becker}, M.~R. and {Bridle}, S.~L. and {Camacho}, H. and {Campos}, A. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Cawthon}, R. and {Chang}, C. and {Chen}, R. and {Chintalapati}, P. and {Crocce}, M. and {Davis}, C. and {Diehl}, H.~T. and {Drlica-Wagner}, A. and {Eckert}, K. and {Eifler}, T.~F. and {Elvin-Poole}, J. and {Everett}, S. and {Fang}, X. and {Fosalba}, P. and {Friedrich}, O. and {Giannini}, G. and {Gruendl}, R.~A. and {Harrison}, I. and {Hartley}, W.~G. and {Herner}, K. and {Huang}, H. and {Huff}, E.~M. and {Huterer}, D. and {Kuropatkin}, N. and {Leget}, P. -F. and {Liddle}, A.~R. and {McCullough}, J. and {Muir}, J. and {Pandey}, S. and {Park}, Y. and {Porredon}, A. and {Refregier}, A. and {Rollins}, R.~P. and {Roodman}, A. and {Rosenfeld}, R. and {Ross}, A.~J. and {Rykoff}, E.~S. and {Sanchez}, J. and {Sevilla-Noarbe}, I. and {Sheldon}, E. and {Shin}, T. and {Troja}, A. and {Tutusaus}, I. and {Varga}, T.~N. and {Weaverdyck}, N. and {Yanny}, B. and {Yin}, B. and {Zhang}, Y. and {Zuntz}, J. and {Aguena}, M. and {Allam}, S. and {Annis}, J. and {Bacon}, D. and {Bertin}, E. and {Bhargava}, S. and {Brooks}, D. and {Buckley-Geer}, E. and {Burke}, D.~L. and {Carretero}, J. and {Costanzi}, M. and {da Costa}, L.~N. and {Pereira}, M.~E.~S. and {De Vicente}, J. and {Desai}, S. and {Dietrich}, J.~P. and {Doel}, P. and {Ferrero}, I. and {Flaugher}, B. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Giannantonio}, T. and {Gschwend}, J. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Hoyle}, B. and {James}, D.~J. and {Kron}, R. and {Kuehn}, K. and {Lahav}, O. and {Lima}, M. and {Lin}, H. and {Maia}, M.~A.~G. and {Marshall}, J.~L. and {Martini}, P. and {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Mohr}, J.~J. and {Morgan}, R. and {Ogando}, R.~L.~C. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Petravick}, D. and {Pieres}, A. and {Plazas Malag{\'o}n}, A.~A. and {Romer}, A.~K. and {Sanchez}, E. and {Scarpine}, V. and {Schubnell}, M. and {Serrano}, S. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Weller}, J.},
        title = "{Dark Energy Survey Year 3 Results: Cosmology from Cosmic Shear and Robustness to Data Calibration}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = may,
          eid = {arXiv:2105.13543},
        pages = {arXiv:2105.13543},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210513543A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{y3-cosmicshear2,
       author = {{Secco}, L.~F. and {Samuroff}, S. and {Krause}, E. and {Jain}, B. and {Blazek}, J. and {Raveri}, M. and {Campos}, A. and {Amon}, A. and {Chen}, A. and {Doux}, C. and {Choi}, A. and {Gruen}, D. and {Bernstein}, G.~M. and {Chang}, C. and {DeRose}, J. and {Myles}, J. and {Fert{\'e}}, A. and {Lemos}, P. and {Huterer}, D. and {Prat}, J. and {Troxel}, M.~A. and {MacCrann}, N. and {Liddle}, A.~R. and {Kacprzak}, T. and {Fang}, X. and {S{\'a}nchez}, C. and {Pandey}, S. and {Dodelson}, S. and {Chintalapati}, P. and {Hoffmann}, K. and {Alarcon}, A. and {Alves}, O. and {Andrade-Oliveira}, F. and {Baxter}, E.~J. and {Bechtol}, K. and {Becker}, M.~R. and {Brandao-Souza}, A. and {Camacho}, H. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Cawthon}, R. and {Cordero}, J.~P. and {Crocce}, M. and {Davis}, C. and {Di Valentino}, E. and {Drlica-Wagner}, A. and {Eckert}, K. and {Eifler}, T.~F. and {Elidaiana}, M. and {Elsner}, F. and {Elvin-Poole}, J. and {Everett}, S. and {Fosalba}, P. and {Friedrich}, O. and {Gatti}, M. and {Giannini}, G. and {Gruendl}, R.~A. and {Harrison}, I. and {Hartley}, W.~G. and {Herner}, K. and {Huang}, H. and {Huff}, E.~M. and {Jarvis}, M. and {Jeffrey}, N. and {Kuropatkin}, N. and {Leget}, P. -F. and {Muir}, J. and {Mccullough}, J. and {Navarro Alsina}, A. and {Omori}, Y. and {Park}, Y. and {Porredon}, A. and {Rollins}, R. and {Roodman}, A. and {Rosenfeld}, R. and {Ross}, A.~J. and {Rykoff}, E.~S. and {Sanchez}, J. and {Sevilla-Noarbe}, I. and {Sheldon}, E.~S. and {Shin}, T. and {Tutusaus}, I. and {Varga}, T.~N. and {Weaverdyck}, N. and {Wechsler}, R.~H. and {Yanny}, B. and {Yin}, B. and {Zhang}, Y. and {Zuntz}, J. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Annis}, J. and {Bacon}, D. and {Bertin}, E. and {Bhargava}, S. and {Bridle}, S.~L. and {Brooks}, D. and {Buckley-Geer}, E. and {Burke}, D.~L. and {Carretero}, J. and {Costanzi}, M. and {da Costa}, L.~N. and {De Vicente}, J. and {Diehl}, H.~T. and {Dietrich}, J.~P. and {Doel}, P. and {Ferrero}, I. and {Flaugher}, B. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Giannantonio}, T. and {Gschwend}, J. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Hoyle}, B. and {James}, D.~J. and {Jeltema}, T. and {Kuehn}, K. and {Lahav}, O. and {Lima}, M. and {Lin}, H. and {Maia}, M.~A.~G. and {Marshall}, J.~L. and {Martini}, P. and {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Mohr}, J.~J. and {Morgan}, R. and {Ogando}, R.~L.~C. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Petravick}, D. and {Pieres}, A. and {Plazas Malag{\'o}n}, A.~A. and {Rodriguez-Monroy}, M. and {Romer}, A.~K. and {Sanchez}, E. and {Scarpine}, V. and {Schubnell}, M. and {Scolnic}, D. and {Serrano}, S. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {Thomas}, D. and {To}, C.},
        title = "{Dark Energy Survey Year 3 Results: Cosmology from Cosmic Shear and Robustness to Modeling Uncertainty}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = may,
          eid = {arXiv:2105.13544},
        pages = {arXiv:2105.13544},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210513544S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{y3-2x2ptbiasmodelling,
        author = {{Pandey}, S. and others},
        title = "{Dark Energy Survey Year 3 Results: Constraints on cosmological parameters and galaxy bias models from galaxy clustering and galaxy-galaxy lensing}",
        year = "2021",
        journal = "To be submitted to MNRAS",
        }

@article{y3-2x2ptmagnification,
        author = {{Elvin-Poole}, J. and others},
        title = "{Dark Energy Survey Year 3 Results: Measurement, modelling and cosmological impact of magnification in galaxy clustering and galaxy-galaxy lensing}",
        year = "2021",
        journal = "To be submitted to MNRAS",
        }

@article{y3-2x2maglimforecast,
	author = {{Porredon}, A. and {Crocce}, M. and {Fosalba}, P. and {Elvin-Poole}, J. and {Carnero Rosell}, A. and {Cawthon}, R. and {Eifler}, T.~F. and {Fang}, X. and {Ferrero}, I. and {Krause}, E. and {MacCrann}, N. and {Weaverdyck}, N. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Amon}, A. and {Avila}, S. and {Bacon}, D. and {Bertin}, E. and {Bhargava}, S. and {Bridle}, S.~L. and {Brooks}, D. and {Carrasco Kind}, M. and {Carretero}, J. and {Castander}, F.~J. and {Choi}, A. and {Costanzi}, M. and {da Costa}, L.~N. and {Pereira}, M.~E.~S. and {De Vicente}, J. and {Desai}, S. and {Diehl}, H.~T. and {Doel}, P. and {Drlica-Wagner}, A. and {Eckert}, K. and {Fert{\'e}}, A. and {Flaugher}, B. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Giannantonio}, T. and {Gruen}, D. and {Gruendl}, R.~A. and {Gschwend}, J. and {Gutierrez}, G. and {Hartley}, W.~G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Hoyle}, B. and {James}, D.~J. and {Jarvis}, M. and {Kuehn}, K. and {Kuropatkin}, N. and {Maia}, M.~A.~G. and {Marshall}, J.~L. and {Menanteau}, F. and {Miquel}, R. and {Morgan}, R. and {Palmese}, A. and {Pandey}, S. and {Paz-Chinch{\'o}n}, F. and {Plazas}, A.~A. and {Rodriguez-Monroy}, M. and {Roodman}, A. and {Samuroff}, S. and {Sanchez}, E. and {Scarpine}, V. and {Serrano}, S. and {Sevilla-Noarbe}, I. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {To}, C. and {Varga}, T.~N. and {Weller}, J. and {Wilkinson}, R.~D.},
	title = "{Dark Energy Survey Year 3 Results: Optimizing the Lens Sample in Combined Galaxy Clustering and Galaxy-Galaxy Lensing Analysis}",
	 journal = {\prd},
	keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
	year = 2021,
	month = feb,
        volume = {103},
	number = {4},
	eid = {043503},
	pages = {043503},
	doi = {10.1103/PhysRevD.103.043503},
	primaryClass = {astro-ph.CO},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201103411P},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{y3-2x2ptaltlensresults,
        author = {{Porredon}, A. and others},
        title = "{Dark Energy Survey Year 3 Results: Cosmological Constraints from Galaxy Clustering and Galaxy-Galaxy Lensing using an Optimized Lens Sample}",
        year = "in prep.",
        journal = "To be submitted to PRD",
        }

@article{y3-3x2ptkp,
         author = {{DES Collaboration}},
        title = "{Dark Energy Survey Year 3 Results: Cosmological Constraints from Galaxy Clustering and Weak Lensing}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = may,
          eid = {arXiv:2105.13549},
        pages = {arXiv:2105.13549},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210513549D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



==> aff.tex <==

$^{1}$ Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA\\
$^{2}$ Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA\\
$^{3}$ Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA\\
$^{4}$ Department of Physics, ETH Zurich, Wolfgang-Pauli-Strasse 16, CH-8093 Zurich, Switzerland\\
$^{5}$ Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK\\
$^{6}$ Laboratoire de Physique de l'Ecole Normale Sup\'erieure, ENS, Universit\'e PSL, CNRS, Sorbonne Universit\'e, Universit\'e de Paris, Paris, France\\
$^{7}$ Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK\\
$^{8}$ Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain\\
$^{9}$ Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain \\
$^{10}$ Argonne National Laboratory, 9700 South Cass Avenue, Lemont, IL 60439, USA\\
$^{11}$ Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA\\
$^{12}$ Physics Department, 2320 Chamberlin Hall, University of Wisconsin-Madison, 1150 University Avenue Madison, WI  53706-1390\\
$^{13}$ Physics Department, 2320 Chamberlin Hall, University of Wisconsin-Madison, 1150 University Avenue Madison, WI  53706-1390\\
$^{14}$ Department of Physics, Northeastern University, Boston, MA 02115, USA\\
$^{15}$ Laboratory of Astrophysics, \'Ecole Polytechnique F\'ed\'erale de Lausanne (EPFL), Observatoire de Sauverny, 1290 Versoix, Switzerland\\
$^{16}$ Department of Physics, Carnegie Mellon University, Pittsburgh, Pennsylvania 15312, USA\\
$^{17}$ California Institute of Technology, 1200 East California Blvd, MC 249-17, Pasadena, CA 91125, USA\\
$^{18}$ Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA 94720, USA\\
$^{19}$ NSF AI Planning Institute for Physics of the Future, Carnegie Mellon University, Pittsburgh, PA 15213, USA\\
$^{20}$ Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{21}$ Department of Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{22}$ Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA\\
$^{23}$ Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA\\
$^{24}$ Faculty of Physics, Ludwig-Maximilians-Universit\"at, Scheinerstr. 1, 81679 Munich, Germany\\
$^{25}$ Department of Physics, University of Oxford, Denys Wilkinson Building, Keble Road, Oxford OX1 3RH, UK\\
$^{26}$ Jodrell Bank Center for Astrophysics, School of Physics and Astronomy, University of Manchester, Oxford Road, Manchester, M13 9PL, UK\\
$^{27}$ Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{28}$ Department of Astronomy/Steward Observatory, University of Arizona, 933 North Cherry Avenue, Tucson, AZ 85721-0065, USA\\
$^{29}$ Department of Physics and Astronomy, Pevensey Building, University of Sussex, Brighton, BN1 9QH, UK\\
$^{30}$ Department of Applied Mathematics and Theoretical Physics, University of Cambridge, Cambridge CB3 0WA, UK\\
$^{31}$ Perimeter Institute for Theoretical Physics, 31 Caroline St. North, Waterloo, ON N2L 2Y5, Canada\\
$^{32}$ Department of Physics, Stanford University, 382 Via Pueblo Mall, Stanford, CA 94305, USA\\
$^{33}$ SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA\\
$^{34}$ Instituto de F\'isica Gleb Wataghin, Universidade Estadual de Campinas, 13083-859, Campinas, SP, Brazil\\
$^{35}$ Brookhaven National Laboratory, Bldg 510, Upton, NY 11973, USA\\
$^{36}$ Department of Physics, Duke University Durham, NC 27708, USA\\
$^{37}$ Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{38}$ Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA\\
$^{39}$ Instituto de F\'{i}sica Te\'orica, Universidade Estadual Paulista, S\~ao Paulo, Brazil\\
$^{40}$ CNRS, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{41}$ Sorbonne Universit\'es, UPMC Univ Paris 06, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France\\
$^{42}$ Center for Astrophysical Surveys, National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA\\
$^{43}$ Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA\\
$^{44}$ Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain\\
$^{45}$ Astronomy Unit, Department of Physics, University of Trieste, via Tiepolo 11, I-34131 Trieste, Italy\\
$^{46}$ INAF-Osservatorio Astronomico di Trieste, via G. B. Tiepolo 11, I-34143 Trieste, Italy\\
$^{47}$ Institute for Fundamental Physics of the Universe, Via Beirut 2, 34014 Trieste, Italy\\
$^{48}$ Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{49}$ Hamburger Sternwarte, Universit\"{a}t Hamburg, Gojenbergsweg 112, 21029 Hamburg, Germany\\
$^{50}$ Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain\\
$^{51}$ Department of Physics, IIT Hyderabad, Kandi, Telangana 502285, India\\
$^{52}$ Department of Astronomy, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{53}$ Institute of Theoretical Astrophysics, University of Oslo. P.O. Box 1029 Blindern, NO-0315 Oslo, Norway\\
$^{54}$ Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain\\
$^{55}$ Institute of Astronomy, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{56}$ Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK\\
$^{57}$ School of Mathematics and Physics, University of Queensland,  Brisbane, QLD 4072, Australia\\
$^{58}$ Center for Astrophysics $\vert$ Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA 02138, USA\\
$^{59}$ Australian Astronomical Optics, Macquarie University, North Ryde, NSW 2113, Australia\\
$^{60}$ Lowell Observatory, 1400 Mars Hill Rd, Flagstaff, AZ 86001, USA\\
$^{61}$ Centre for Gravitational Astrophysics, College of Science, The Australian National University, ACT 2601, Australia\\
$^{62}$ The Research School of Astronomy and Astrophysics, Australian National University, ACT 2601, Australia\\
$^{63}$ Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{64}$ George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA\\
$^{65}$ Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA\\
$^{66}$ Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain\\
$^{67}$ Department of Astronomy, University of California, Berkeley,  501 Campbell Hall, Berkeley, CA 94720, USA\\
$^{68}$ School of Physics and Astronomy, University of Southampton,  Southampton, SO17 1BJ, UK\\
$^{69}$ Computer Science and Mathematics Division, Oak Ridge National Laboratory, Oak Ridge, TN 37831\\
$^{70}$ Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany\\
$^{71}$ Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany


==> results.tex <==
% All content moved to main.tex

==> tables.tex <==












